The maximum four point condition matrix of a tree

$\newcommand{\Max}{\mathrm{Max4PC}}$ The Four point condition (4PC henceforth) is a well known condition characterising distances in trees $T$. Let $w,x,y,z$ be four vertices in $T$ and let $d_{x,y}$ denote the distance between vertices $x,y$ in $T$. The 4PC condition says that among the three terms $d_{w,x} + d_{y,z}$, $d_{w,y} + d_{x,z}$ and $d_{w,z} + d_{x,y}$ the maximum value equals the second maximum value. We define an $\binom{n}{2} \times \binom{n}{2}$ sized matrix $\Max_T$ from a tree $T$ where the rows and columns are indexed by size-2 subsets. The entry of $\Max_T$ corresponding to the row indexed by $\{w,x\}$ and column $\{y,z\}$ is the maximum value among the three terms $d_{w,x} + d_{y,z}$, $d_{w,y} + d_{x,z}$ and $d_{w,z} + d_{x,y}$. In this work, we determine basic properties of this matrix like rank, give an algorithm that outputs a family of bases, and find the determinant of $\Max_T$ when restricted to our basis. We further determine the inertia and the Smith Normal Form (SNF) of $\Max_T$.

==> inertia.tex <==

\section{Inertia of $\Max_T$}

In this Section, we determine the Inertia of $\Max_T$. For an 
$n\times n$ real symmetric matrix $A$, we denote its number 
of positive, negative and zero eigenvalues by $n_+$, $n_-$
and $n_0$, respectively. Recall that the inertia of $A$, 
denoted $\text{Inertia}(A)$, is the triple $(n_0, n_+, n_-)$.


\begin{theorem}
\label{thm:inertia_max4pc}
Let $T$ be a tree on $n$ vertices with $p$ many leaves. Then signature of $\Max_T$ is 
$$
(n_0,n_+,n_-) = \left(\binom{n}{2}-2(n-p),\: n-p,\: n-p\right).
$$
\end{theorem}

\begin{proof}
	The result follows by applying induction on $n$. First notice that if we two leaves $u$ and $v$ of $T$ have a common neighbors then by Lemma \ref{lem:remove extra leaf}, we have
	$$
	\rank(\Max_T) =\rank(\Max_{T-u})=\rank(\Max_{T-v}).
	$$
	The results by applying induction hypothesis on the tree $T-u$.
	
	Now we assume that every quasi-pendant vertex is adjacent to exactly one leave.  Let $\BB$ be a basis of the row space of $\Max_T$ as described in Remark \ref{rem:algo}. Without loss of generality assume that $n$ is a leave adjacent to $n-1$ with $\deg(n-1)=2$. Suppose $n-2\sim n-1$. Then $\{n,n-1\}$ and $\{n,n-2\}$ is in $\BB$. Further, $\widehat{\BB}=\BB\setminus\{\{n,n-1\}, \{n,n-2\}\}$ is a basis of $\Max_{T-n}$. It follows that $\Max_{T}[\BB,\BB]$ is similar to
	$$
	\begin{bmatrix}
		\Max_{T-n}[\widehat{BB},\widehat{BB}] & \0\\
		\0 & \begin{bmatrix}
			0&2\\2&0
		\end{bmatrix}
	\end{bmatrix}.
	$$
	Hence, the result follows by applying Sylvester’s law of inertia and induction hypothesis. 
\end{proof}


\begin{theorem}
Let $T$ be the star tree on $n$ vertices. Then, we have 
$$
\det(xI-\Max_T) = x^{\binom{n}{2}-2}\left(x^2-2(n-1)^2x-	(n-1)-\binom{n-1}{2}\right),
$$
and the nonzero eigenvalues of $\Max_T$ are 
$$
(n-1)^2 \pm \sqrt{(n-1)^4+ (n-1)\binom{n-1}{2}}.
$$
\end{theorem}

\begin{proof}
	Clearly, $\rank(\Max_T)=2$. Let $\lambda$ and $\mu$ be two nonzero eigenvalues of $\Max_T$. Now note that 
	$$
	\Max_T = \begin{bmatrix}
		2J_{(n-1)\times (n-1)} & 	3J_{(n-1)\times \binom{n-1}{2}}\\
		3J_{\binom{n-1}{2}\times (n-1)} & 	4J_{\binom{n-1}{2}\times \binom{n-1}{2}}
	\end{bmatrix}.
	$$
	Therefore, $\lambda+\mu = 2(n-1)+2(n-1)(n-2) = 2(n-1)^2$. Further, note that the sum all  $2\times 2$  principal minors of $\Max_T$ is 
	$
	- (n-1)+\binom{n-1}{2}
	$. It follows that 
	$$
	\lambda\mu = -(n-1)-\binom{n-1}{2}.
	$$
	Therefore, the characteristic polynomial of $\Max_T$ is given by 
	$$
x^{\binom{n}{2}-2}\left(x^2-2(n-1)^2x-	(n-1)-\binom{n-1}{2}\right).
	$$ 
	This completes the proof.
\end{proof}


